Density Decomposition in Dual-Modular Optimization: Markets, Fairness, and Contracts

We study a unified framework for optimization problems defined on dual-modular instances, where the input comprises a finite ground set $V$ and two set functions: a monotone supermodular reward function $\f$ and a strictly monotone submodular cost function $\g$. This abstraction captures and generalizes classical models in economics and combinatorial optimization, including submodular utility allocation (SUA) markets and combinatorial contracts. At the core of our framework is the notion of density decomposition, which extends classical results to the dual-modular setting and uncovers structural insights into fairness and optimality. We show that the density decomposition yields a canonical vector of reward-to-cost ratios (densities) that simultaneously characterizes market equilibria, fair allocations -- via both lexicographic optimality and local maximin conditions -- and best-response strategies in contract design. Our main result proves the equivalence of these fairness notions and guarantees the existence of allocations that realize the decomposition densities. Our technical contributions include the analysis of a broad family of convex programs -- parameterized by divergences such as quadratic, logarithmic, and hockey-stick functions -- whose minimizers recover the density decomposition. We prove that any strictly convex divergence yields the same canonical density vector, and that locally maximin allocations act as universal minimizers for all divergences satisfying the data processing inequality. As an application of our framework, we determine the structure and number of critical values in the combinatorial contracts problem. Additionally, we generalize a Frank-Wolfe-type iterative method for approximating the dual-modular density decomposition, establishing both convergence guarantees and practical potential through efficient gradient oracle design.

==> program.tex <==

\section{Intuition and Technical Overview}
\label{sec:intuition}


\noindent \textbf{Generalization to Submodular $\g$.}
each $u \in V$ does not receive a fixed contribution from $\g$.
For a general submodular function~$\g$,
In the literature, the base polymatroid is considered:

$$\mcal{B}^{\leq}_\g := \{y \in \Delta_\g(V):
\forall S \subseteq V, y(S)  \leq \g(S)\}.$$

Similar to Fact~\ref{fact:perm_polytope},
the polytope $\mcal{B}^{\leq}_\g$ is the convex hull
of $\g^\sigma$ over $\sigma \in \mcal{S}_V$.



A natural way for extending the convex program in Fact~\ref{fact:convex_density}
is to replace the fixed $\g_u$ for linear $\g$ by
a variable vector $y \in \mcal{B}^{\leq}_\g$.  
This would immediately give the following convex program:


\begin{align*}
\min\quad \sum\limits_{u\in V} y_u \cdot (\frac{x_u}{y_u})^2  &\\
x \in \mcal{B}^{\geq}_\f,
y  \in \mcal{B}^{\leq}_\g &
\end{align*}




\noindent \emph{More General Objective Functions.}
As observed in the literature~\cite{?????},
instead of $x \mapsto x^2$,
one can use a general %differentiable 
strictly convex function
$\vartheta: \R_{\geq 0} \to \R$ in the objective function,
i.e., for $0 \leq x < y$
and $0 < \lambda < 1$,
$\vartheta(\lambda x + (1-\lambda) y) < \lambda \vartheta(x) 
+ (1 - \lambda) \vartheta(y)$.
%$\vartheta'(x) < \vartheta'(y)$.
The objective function can be expressed in terms of a general divergence
between distributions.  To ease the description, 
we focus on the normalized case $\f(V) = \g(V) = 1$.

\begin{definition}[$\vartheta$-Divergence]
\label{defn:div}
Given a convex function~$\vartheta$,
the $\vartheta$-divergence between two
distributions $x, y$ in $\Delta(V)$ is defined as:

$$\D_\vartheta(x \| y) := \sum_{u \in V} y_u \cdot \vartheta(\frac{x_u}{y_u}),$$

\end{definition}


\noindent \textbf{Notation Convention.}
When $y$ has zero coordinates,
we use the convention that (i) $0 \cdot \vartheta(\frac{0}{0}) = 0$, 
and (ii) for $a > 0$, $0 \cdot \vartheta(\frac{a}{0}) = a \lim_{x \to + \infty} \frac{f(x)}{x}$.  





We consider the following general convex program.


\ignore{
\begin{definition}[Distribution of Permutations]
{Let $\Delta(\mathcal{S}_V):=\{(p_{\sigma})_{\sigma\in \mathcal{S}_V}: \sum_{\sigma\in \mathcal{S}_V}p_{\sigma}=1, p_{\sigma}\geq 0  \text{ }\forall \sigma\in \mathcal{S}_V \}$ denote the collection of all distributions of permutations. Furthermore, $\vecp:=(p_{\sigma})_{\sigma\in \mathcal{S}_V}\in \Delta(\mathcal{S}_V)$ denotes a distribution of permutations.}
\end{definition}
}


\begin{definition}[General Convex Program]
\label{defn:general_convex}
Given an input instance $(V; \f,\g)$ as in Definition~\ref{defn:input} and 
a differentiable strictly convex function $\vartheta: \mathbb{R}_{\geq 0}\rightarrow \mathbb{R}$,
define the following convex program:


\begin{align*}
\min\quad \D_\vartheta(x \| y)  &\\
x \in \mcal{B}^{\geq}_\f,
y  \in \mcal{B}^{\leq}_\g &
\end{align*}


In view of Fact~\ref{fact:perm_polytope},
we will have an equivalent formulation in terms of permutation distributions:


\begin{align*}
 \mathsf{CP:}\min\quad \Phi(\vecp, \vecq) &:= \D_\vartheta(\f^{\vecp} \| \g^{\vecq})  \\
%\text{s.t.}\quad \rho_u &= \frac{\f^{\vecp}_u}{\g^{\vecp}_u}  & \forall u\in V \\
%\sum_{\sigma\in \mathcal{S}_V}\g_{\sigma}(u)\cdot p_{\sigma} &=\g_u&\forall u\in V\\
%{\f_u}\cdot{\g_u}^{-1}&=\rho_{u}&\forall u\in V\\
\vecp, \vecq &\in \Delta(\mathcal{S}_V) 
\end{align*}


We also denote the induced density vector $\rho^{(\vecp, \vecq)} \in \R^V$,
where $\rho^{(\vecp, \vecq)}(u) = \frac{\f^{\vecp}_u}{\g^{\vecq}_u}$,
for $u \in V$.



\ignore{
We also denote the induced density vector $\rho^{(\vecp, \vecq)} \in \R_*^V$,
where $\R_* := \R \cup \{\bot, +\infty\}$,
as follows:

for $u \in V$,
 $\rho^{(\vecp, \vecq)}(u) =  
\begin{cases}
\bot, & \text{if } \f^{\vecp}_u = \g^{\vecq}_u = 0; \\
\frac{\f^{\vecp}_u}{\g^{\vecq}_u}, & \text{otherwise.}
\end{cases}
$

We denote $V^{(\vecp, \vecq)} := \{u \in V: \rho^{(\vecp, \vecq)}(u) \neq \bot\}$.
}
%Furthermore, define $\alpha_{\f}:=(\f_u)_{u\in V}$, $\alpha_{\g}:=(\g_u)_{u\in V}$ and $\rho:=(\rho_u)_{u\in V}$ and let $\{\vecp,\alpha_{\f},\alpha_{\g},\rho\}$ denote the feasible solution to the convex program.
\end{definition}

\begin{remark}
The objective function in Definition~\ref{defn:general_convex}
is convex because for any $c, d \in \R^m$,
the function $(x, y) \in \R^m \times \R^m \mapsto \langle d, y \rangle \cdot \vartheta(\frac{\langle c, x \rangle}{\langle d, y \rangle })$
is convex due
to property of \emph{perspective functions}~\cite{CVOP}.
\end{remark}


\noindent \textbf{Extra Equality Constraint.}
We later show that the minimum of the convex program $\mathsf{CP}$ in 
Definition~\ref{defn:general_convex}
can be attained with an extra equality constraint $\vecp = \vecq$.
Hence, when there is no ambiguity, we will overload
the notation $\Phi(\vecp) :=  \Phi(\vecp, \vecp)$
and $\rho^{\vecp} := \rho^{(\vecp, \vecp)}$.

\noindent \textbf{Compact Solution Representation.}
Even though the convex program $\Phi(\vecp)$ in Definition~\ref{defn:general_convex}
has an exponential number of variables in $\vecp$,
it suffices to maintain the corresponding $\f^{\vecp}$ and 
$\g^{\vecp} \in \R^V$ in an iterative algorithm.
We give the generalization of Algorithm~\ref{alg:abstract} as follows.




\begin{algorithm}[H]
\caption{General Abstract Iterative Procedure}\label{alg:general_abstract}
\begin{algorithmic}[1]
\State \textbf{Input:} Supermodular $\f : 2^V \to \R$; submodular $\g: 2^V \to \R$;
step size $\gamma: \Z_{\geq 0} \to [0,1]$;
number $T$ of iterations.

\State    \text{\textbf{Initialize}:} Pick an arbitrary permutation $\sigma_0 \in \mcal{S}_V$;
set $(f^{(0)}, g^{(0)}) \gets (\f^{\sigma_0}, \g^{\sigma_0}) \in \R^V \times \R^V$.

 
 
\For{ $k \gets 0 \text{ to } T-1$}

 %\State $\gamma \gets \frac{1}{k+1}$
		
		\State $\sigma_{k+1} \gets \textsc{Abstract-Perm}(\f, \g, \gamma_k, f^{(k)}, g^{(k)})$
		\label{ln:abstract_perm}
		
		\State $(c^{(k+1)}, d^{(k+1)}) \gets (\f^{\sigma_{k+1}}, \g^{\sigma_{k+1}})$
		
		
     \State $(f^{(k+1)}, g^{(k+1)}) \gets (1 - \gamma_k) \cdot (f^{(k)}, g^{(k)})+\gamma_k \cdot (c^{(k+1)}, d^{(k+1)})$ \label{ln:update2}
 
\EndFor
\State \text{\textbf{return: $(f^{(T)}, g^{(T)}) \in \R^V \times \R^V$} }  
\end{algorithmic}
\end{algorithm}


\noindent \textbf{Intuition.}
To instantiate a variant of Algorithm~\ref{alg:general_abstract},
it suffices to specify the step size function~$\gamma$
and how to implement \textsc{Abstract-Perm} to return an appropriate
permutation of $V$.  A natural way is to sort the elements $u$ in $V$ according 
to some score metric.  Following the case for linear $\g$,
given a solution $\vecp \in \Delta(\mcal{S}_V)$,
one can consider $\rho^{\vecp}(u)$ for $u \in V$.
To this end, we define a \emph{local maximin} condition for a solution,
variants of which have appeared in the literature~\cite{???????}.

\begin{definition}[Local Maximin]
\label{defn:local_maximin}
Given an instance $(V; \f, \g)$,
a solution $(\vecp, \vecq) \in \Delta(\mcal{S}_V)^2$
is locally maximin if for all $u, v \in V$
such that $\rho^{(\vecp, \vecq)}(u) > \rho^{(\vecp, \vecq)}(v)$
(where we use the convention that $a > \bot$ for $a \neq \bot$)
and 
$\sigma \in \mcal{S}_V$ such that $p_\sigma > 0$ or $q_\sigma > 0$,
it holds that $u \prec_\sigma v$.


\end{definition}






\noindent \textbf{Technical Roadmap.}  Following the intuition of 
our approach, we will formalize the results subsequently.
\begin{enumerate}

\item We will show that any optimal solution $\vecp$ to the convex program
in Definition~\ref{defn:general_convex}
induces the same density vector $\rho^{\vecp} = \rho^*$ given
by the density decomposition in Definition~\ref{defn:density_decomp}.
However, note that an optimal distribution $\vecp$ of permutations for the convex program
needs not be unique.

\item We will show how to instantiate a variant
of Algorithm~\ref{alg:general_abstract}
that is equivalent to applying the Frank-Wolfe algorithm
to the general convex program.

Similar to the special case, we pick the step size
$\gamma_k := \frac{2}{k+2}$.  Moreover,
to implement \textsc{Abstract-Perm},
given some current $(f^{(k)}, g^{(k)}) \in \R^V \times \R^V$,
we show that it suffices to 
sort the elements~$u \in V$
in non-increasing order of
$\rho^{(k)}_u := \frac{f^{(k)}_u}{g^{(k)}_u}$
to produce the desired permutation.


\item Given that some solution satisfies
$\Phi(\vecp^{(T)}) - \Phi(\vecp^*) \leq \epsilon$,
we will derive an upper bound
for the norm of the difference between the corresponding density vectors $\|\rho^{(T)} - \rho^*\|$.

\hubert{Lemma 8.4 in symmetric splendor paper}

\end{enumerate}




==> reference.tex <==
\section*{}
\bibliographystyle{plain}
\bibliography{ref}


\addcontentsline{toc}{section}{References}
\begin{thebibliography}{99}
\bibitem{a} Satoru Fujishige, \emph{Submodular Functions and Optimization}, Elsevier Science \& Technology, 2005.
\bibitem{b} Harb Elfarouk, Quanrud Kent, Chekuri Chandra, \emph{Faster and Scalable Algorithms for Densest Subgraph and Decomposition}, NeurIPS 2022.
\bibitem{c}Maximilien Danisch, T.-H. Hubert Chan, and Mauro Sozio, \emph{Large scale density-friendly graph decomposition via convex programming}, WWW17, page 233–242.
 \bibitem{d}Chandra Chekuri, Shalmoli Gupta, and Kent Quanrud, \emph{Streaming algorithms for
submodular function maximization}, In: Automata, Languages, and Programming:
42nd International Colloquium, ICALP 2015, Kyoto, Japan, July 6-10, 2015, Proceedings, Part I 42
\bibitem{e}Chandra Chekuri, Kent Quanrud and Manuel R. Torres, \emph{Densest Subgraph: Supermodularity, Iterative Peeling, and Flow}, SODA22
\bibitem{f}Chandra Chekuri, Elfarouk Harb and Kent Quanrud, \emph{Convergence to Lexicographically Optimal Base in a (Contra)Polymatroid and Applications to Densest Subgraph and Tree Packing}, ESA22
\bibitem{g}Martin Jaggi. \emph{Revisiting Frank-Wolfe: Projection-free sparse convex optimization}, In Sanjoy Dasgupta and David McAllester, editors, Proceedings of the 30th International Conference on Machine Learning, number 1 in Proceedings of Machine Learning Research, pages 427–435, Atlanta, Georgia, USA, 17–19 Jun 2013. PMLR.
\bibitem{h} {Boyd Stephen and Vandenberghe Lieven}, \emph{Convex optimization}, page 90, {Cambridge university press},{2004}.


\end{thebibliography}

==> related_work.tex <==


\newpage
\section{Related Work}

Submodular(Supermodular)-Linear References:
\begin{itemize}

\item{density:   ~\cite{DBLP:journals/csur/LancianoMFB24}~\cite{DBLP:conf/soda/ChekuriQT22}~\cite{DBLP:conf/nips/HarbQC22} ~\cite{DBLP:conf/esa/HarbQC23}
These papers consider the densest subgraph problem with respect to density defined by $$\rho(S)=\frac{f(S)}{g(|S|)}$$ where $f$ is monotone supermodular and $g$ is concave








~\cite{DBLP:conf/isaac/KawaseM16a}

This paper considers the densest subgraph problem with respect to density defined by $$\rho(S)=\frac{w(S)}{f(|S|)}$$ where $f$ is convex and $g$ is linear.




}


\item{contract:
~\cite{DBLP:conf/focs/DuttingEFK21}. This is already shown in the paper.}

\item{tree packing:  ~\cite{DBLP:conf/esa/HarbQC23}~\cite{DBLP:conf/stoc/Thorup08}


Consider a connected multi-graph $G = (V, E)$ with $n$ vertices and $m$ edges. Let $M_{G}(E, F)$ be the graphic matroid  induced by $G$, where $E$ is the ground set and $F$ consists of all sub-forests of $G$. The bases of the matroid
are given by the spanning trees of $G$. Consider the rank function $r: 2^{E}\rightarrow \mathbb{Z}_{\geq 0}$ of $M_G$. Note that $r$ is submodular and for a edge subset $X \subseteq E$, $r(X) = n - \kappa(X)$ where $\kappa(X)$ is the number of connected components induced by $X$. The following problem is equivalent to the usual density decomposition problem, $$\min_{S\subseteq E}\frac{|E|-|S|}{f(E)-f(S)}$$





}



\item{Market:
~\cite{DBLP:journals/geb/JainV10}~\cite{DBLP:conf/ipco/Nagano07}~\cite{Panditi2016}

These are already mentioned in the introduction.}

\item{Sparsification: ~\cite{DBLP:conf/soda/Quanrud24a}

Given monotone submodular function $f$ and nonnegative weights $w$ which are both defined on the subsets of a finite set $\mathcal{N}$, the paper takes advantage of the quantity $${\varphi}(S)=\frac{w(\mathcal{N})-w(S)}{f(\mathcal{N})-w(S)}$$ to sparsify the weight of every quotient of $f$.



}

\item{Online Assigment (Water Level): ~\cite{DBLP:conf/focs/HathcockJPSZ24}

Given a ground set $E$ and a monotone submodular function $f$, for an allocation $x\in \mathbb{R}_{\geq 0}^{E}$, the paper defined a water level vector $w^{(x)}$ as follows to derive a water-level type algorithm to solve the online assignment problem.$$w_{e}^{(x)}=\max\limits_{e\in S}\min\limits_{\substack{T\subseteq E \\f_{T}(\{e\})\neq 0}}\frac{x(S\setminus T)}{f(S\cup T)-f(T)}$$
}

\item{Matroid Intersection Market:~\cite{DBLP:conf/soda/BuchbinderGHKS24}
Given an arbitrary matroid $M=(E, I)$ and a partition matroid $P$ on the elements in $E$, the paper define the inverse expansion of a set of buyers as $$InvExp_{M}(B')=\frac{m(B')}{rank_{M}(N(B'))}$$
where $m(B')=\sum_{i\in B'}m_i$ is the budget of a subset of buyers and $N(B')=\bigcup_{i\in B'}P_i$ is the neighborhood of these buyers as all elements in all of their parts. The authors give an algorithm to output a nested family of elements in $E$ which is called the matroid intersection skeleton via the above quantity.


}



\end{itemize}
